On the Limitations of Cross-lingual Encoders as Exposed by Reference-Free Machine Translation Evaluation

Evaluation of cross-lingual encoders is usually performed either via zero-shot cross-lingual transfer in supervised downstream tasks or via unsupervised cross-lingual textual similarity. In this paper, we concern ourselves with reference-free machine translation (MT) evaluation where we directly compare source texts to (sometimes low-quality) system translations, which represents a natural adversarial setup for multilingual encoders. Reference-free evaluation holds the promise of web-scale comparison of MT systems. We systematically investigate a range of metrics based on state-of-the-art cross-lingual semantic representations obtained with pretrained M-BERT and LASER. We find that they perform poorly as semantic encoders for reference-free MT evaluation and identify their two key limitations, namely, (a) a semantic mismatch between representations of mutual translations and, more prominently, (b) the inability to punish "translationese", i.e., low-quality literal translations. We propose two partial remedies: (1) post-hoc re-alignment of the vector spaces and (2) coupling of semantic-similarity based metrics with target-side language modeling. In segment-level MT evaluation, our best metric surpasses reference-based BLEU by 5.7 correlation points.

==> 1-introduction_old.tex <==
\section{Introduction}

%%%%%%%%%%%%%%%
%GG: Mismatch between the nature of the text generation tasks and the classic fixed-label-set evaluation setup 
%%%%%%%%%%%%%%%

Standard evaluation setup for supervised machine learning (ML) tasks assumes an evaluation metric that compares a set of model's predictions with a set of gold labels to a classifier prediction.\footnote{In settings where collecting gold labels is notoriously difficult, different evaluation paradigms are arguably more suitable---e.g., evaluating classifier's performance by comparing its predictions to predictions of a multitude of other classifiers  \citep{Platanios:2016:EAU:3045390.3045540}}\todo{SE: I don't understand this sentence. The standard case is single-label classification, i.e., comparing a classifier prediction to a gold label. Does this talk here about multi-label classification? But even so, I wouldn't understand.} This standard evaluation setup, which dominates the evaluation landscape of natural language processing (NLP) as well has one major assumption: that the task comes with a set of clearly defined and unambiguous labels and, in most cases, that an instance can be assigned few labels.\todo{SE: you mean multi-label classification or the size of the label set is small?} This assumption, however, does not hold for text generation tasks like machine translation (MT) \cite{bahdanau2014neural,johnson2017google} and text summarization \cite{rush2015summarization,tan2017abstractive}, where we do not predict a single discrete label but rather generate natural language text. Since natural language is by definition ambiguous and unconstrained, the set of labels for text generation tasks is neither clearly defined nor finite. Yet, the standard evaluation protocols for text generation tasks still follow the described default paradigm: (1) evaluation datasets come with human-created reference texts (i.e., translations and summaries written by humans) and (2) evaluation metrics, e.g., BLEU \cite{Papineni:2002} or METEOR \cite{lavie2007meteor} for MT and ROUGE \cite{lin2003automatic} for summarization, count the exact ``label'' (i.e., n-gram) matches between the reference text and system-generated text. In other words, established text generation evaluation compares semantically ambiguous and imprecise labels from an unbounded set (i.e., natural language texts) via crisp symbolic matching (i.e., string overlap).   

%%%%%%%%%%%%%%%
%GG: Next we mention the monolingual "semantic" comparison approaches: these remove the "crisp symbolic comparison" problem and allow for semantic comparison, but do not remove the fact that we're comparing the generation with only one of very many possible/correct reference texts. And still require reference text (costly annotation effort) -- reference-free metrics remedy for this.   
%%%%%%%%%%%%%%%
The first remedy is to replace the crisp symbolic comparison of natural language ``labels'' with the comparison of texts' meaning, which requires reference texts and system generations to be embedded into the same latent semantic space. Recently, a number of MT evaluation methods appeared focusing on semantic comparison of reference translations and system translations \cite{Shimanaka:2018,clark-etal-2019-sentence,zhao2019moverscore}. While these metrics demonstrate higher correlation than n-grap overlap metrics like BLEU or METEOR with human assessments of semantic alignment between reference and system translations, they do not address the issues inherent to having reference translations. Namely, that (1) reference translations are expensive to obtain and (2) a reference translation assumes a single correct solution and biases the evaluation, both automatic and human \cite{dreyer2012hyter,fomicheva2016reference}.\todo{SE: I think in summarization, people use multiple references}        

%%%%%%%%%%%%%%%
%GG: Now motivating reference-free MT evaluation metrics    
%%%%%%%%%%%%%%%
Reliable reference-free evaluation metrics, directly measuring the (semantic) correspondence between the source language text and the system translation, would remove the need for human reference translations in MT evaluation and allow for MT evaluations much wider in scope: besides for training MT models, any parallel corpus could also directly be used for evaluating the MT systems.\todo{SE: everything after the colon, I don't understand} Yet, the proposals of reference-free MT evaluation metrics have been few and far apart\todo{SE: in time?} and have required either non-negligible supervision (i.e., human translation quality labels) \cite{specia2010machine} or language-specific preprocessing like semantic parsing \cite{lo-2014-xmeant,lo-2019-yisi}, both hindering the wide applicability of the proposed metrics.

%%%%%%%%%%%%%%%
%GG: Now our contributions
%%%%%%%%%%%%%%%
In this work, we comparatively evaluate a number of reference-free MT evaluation metrics that rely on the most recent developments in multilingual representation learning, namely cross-lingual (static and contextualized) embeddings \cite{conneau2018word,devlin2019bert} and multilingual sentence encoders \cite{artetxe2019massively,yang2019multilingual}, and require no supervision nor any language-specific preprocressing.\todo{SE: we require no supervision? Except when we post-align MBERT?} We investigate two types of cross-lingual reference-free metrics. \textbf{(1)} \textit{Soft token-level alignment} metrics find the optimal soft alignment between source sentence and system translation token using %the 
Word Mover's Distance (WMD) \cite{kusner2015word}. \newcite{zhao2019moverscore} recently demonstrated that WMD, operating on BERT-contextualized \todo{SE: BERT-contextualized?} significantly outperforms  baseline MT evaluation metrics, in the monolingual reference-based setting. Here, we investigate whether WMD can be similarly successful useful in the cross-lingual (i.e., reference-free) setup, applied on top of cross-lingual token representations. \textbf{(2)} \textit{Sentence-level similarity} metrics measure the similarity between sentence representations of the source sentence and system translation, as produced by multilingual sentence encoders like LASER \cite{artetxe2019massively} and USE \cite{cer-etal-2018-universal,yang2019multilingual}. 

Our analysis yields several interesting findings. We show that, unlike in the monolingual reference-based setup \cite{zhao2019moverscore}, the cross-lingual reference-free evaluation metrics fail to outperform the reference-based baseline metrics like BLEU.
\todo{YG: even in monolingual setup, reference-free metrics underperform reference-based ones, don't they? The MoverScore paper does not study any reference-free metrics.}
We identify the inability of both above classes of cross-lingual metrics to capture and punish ``translationese'', i.e., literal word-by-word translations of the source sentence. We next show that there is still a significant language bias in the cross-lingual representations produced by state-of-the semantic encoders like Multilingual BERT \cite{devlin2019bert} and LASER \cite{artetxe2019massively} (vectors of mutual translations are insufficiently close) and that by executing an additional weakly-supervised cross-lingual alignment step, we can improve the performance of all reference-free metrics under investigation. Finally, we show that the combination of cross-lingual reference-free metrics and language modeling on the target side (which is able to detect ``translationese''), surpasses the performance of strong reference-based baselines. We believe these findings indicate web-scale domain-agnostic MT evaluation (i.e., MT evaluation ``in the wild'') a viable prospect, which is particularly
promising for low-resource languages, which lack large amounts of parallel data.\todo{SE: the intro appears too long, by about 1/2-1 page}
 

%We show that both of these model classes have undesirable shortcomings which allow for `fooling' them: for example, they are indifferent between high-quality human references and very low-quality word-by-word translations of a source language sentence.

%concern ourselves with the recently emerging field of \emph{reference-free} machine translation evaluation.\footnote{Take WMT shared tasks as evidence, starting from WMT2018 or WMT2019, I think} Our contributions are as follows:
%\begin{enumerate}
    %\item 
%    (1) We investigate reference-free MT evaluation using cross-lingual sentence encoders \cite{artetxe2019massively} and adaptations of recent models using contextualized word embeddings \citep{zhao2019moverscore} to the cross-lingual setting. 
%{\color{red}{Wei's original text:}}

%(2)  %which we frame in the context 
%    This hitherto undetected phenomenon, which challenges the usability of cross-lingual encoders at large scale, has particularly severe consequences for reference-free MT evaluation, as it will lead to evaluation metrics falsely claiming superiority of low-performing MT systems. 
%    We frame this deficit as a `bias' \citep{} and apply recently proposed debiasing techniques along with target language based language models to address them. 
%    (3) By combining these techniques, we achieve a reference-free MT evaluation model which outperforms strong \emph{reference-based} baselines such as BLEU and even rivals \emph{supervised reference-based} baselines\footnote{Trained on human scores as supervision signal.} such as XX.  
%    \todo[inline]{SE: frame DA$=$CLDA as a contribution?}
%\end{enumerate}

%\todo[inline]{SE: the table with supervised/unsupervised on both axes?}


% summarization texts 

%% GG: that annotating data is costly is a well known fact, I wouldn't emphasize it this much. 

%A couple of fundamental implications go along with this basic tenet, e.g., that system evaluation is tied to specifically labeled datasets, which are  low-resource in nature, as labeling data is costly.
%\todo[inline]{Could use crowds or distant supervision}
%Evaluating on little labeled data, in turn, brings with it the risk of falsely assessing classifier performance, which is particularly true when the data on which the trained system will subsequently be applied follows a distribution different from the one on which it has been trained (domain shift). 
  

%, with  in ML, %With 
%despite a 
%with only few isolated exceptions---e.g., evaluating classifier performance by comparing it to a multitude of other classifiers' predictions \citep{Platanios:2016:EAU:3045390.3045540}. %---

%comparing predictions to ground truth labels is still by far the dominating paradigm in all of supervised machine learning, including the paradigms in natural language processing (NLP).
%this paradigm 

%Implied by this assumption is  
%This basic tenet has 

%For some tasks in natural language processing (NLP), like text generation problems such as machine translation \citep{} or summarization \citep{} this evaluation paradigm appears somewhat less justified than for traditional ML classification problems, as their  `labels' are generated pieces of text, just like the inputs. Comparing two pieces of text is, however, a much %comparatively 
%simpler and more well-established NLP problem than 
%, much easier 
%than 
%comparing an input text to an `artificial' class label. 
%Still, so called \emph{reference-free} text generation evaluation has rarely been addressed in the literature before (as exceptions consider e.g.\ \citet{}), and most approaches to evaluation of machine translation, our focus in this work, or summarization are based on comparing system outputs to human gold references, just as in the classical ML setting \citep{}. This is true for both 
%
%traditional MT evaluation, %has used the so-called BLEU score \cite{}, which compares 
%which uses BLEU scores to compare $n$-grams in  system translations to those in human references   %While BLEU has dominated the field %of MT evaluation 
%for almost two decades now and is (probably) still the most reported evaluation metric as of 2019, it is well-known for its deficits, such as its inability to distinguish between high performing systems and its low correlations (at segment level) with human assessments \citep{}. \todo[inline]{SE: list more}. In the recent 1 to 2 years, with the advent of contextualized word embeddings, 
%and 
%the variety of novel MT evaluation metrics, based on contextualized word embeddings \citep{}, which have recently been proposed and which address %majority  of shortcomings , in particular, the 
%an array of shortcomings of lexical-based metrics such as their 
%low correlations with human assessments \citep{}. 
%However, these metrics still use costly human references and are therefore limited to those domains for which (high-quality) parallel data is available. 

% \begin{figure}
% \centering
% \includegraphics[width=200pt]{figures/concept.pdf}
% \caption{Toy example of }
% \end{figure}

==> 3-approach_old.tex <==
\section{Reference-Free MT Evaluation Metrics }
%In this work, we %abstract away 
%free ourselves 
%from the need for costly human references in MT evaluation by introducing a ``reference-free'' metric. We now describe our metric in detail.
% named XMoverScore that can be seen as a variant of MoverScore~\cite{DBLP:conf/emnlp/no_reference19}.

% cross-lingual variant of MoverScore.
% using cross-lingual metric.
% replacing the monolingual word embeddings in MoverScore with cross-lingual embeddings~\cite{lample2019cross,Artetxe:2018}. 

% investigate three approaches to compare neural and non-neural MT systems in reference-free condition: 

% Let $\bx$ and $\by$ be two sentences viewed as sequences of $n$-grams: $\bx^n$ and $\by^n$.
% be source sentence viewed as a sequence of words. We denote by $\bx^n$ the sequence %list 
% of $n$-grams of $\bx$ (i.e., $\bx^1=\bx$ is the sequence %list 
% of words and $\bx^2$ is the sequence of bigrams).
%\subsection{Notation}
In the following, we use $\mathbf{x}$ to %refer to 
denote a source sentence (i.e., a sequence of tokens in 
the source language),
%tokens) 
$\mathbf{y}$ to denote a system translation of $\mathbf{x}$ in the 
target language, 
and $\mathbf{y}^\star$ to denote the human-written
reference translation for $\mathbf{x}$. 
%Thus, we have triples $(\mathbf{x},\mathbf{y},\mathbf{y}^\star)$. 
%YG: why we have y^star? aren't we study ref-free metric? if use DA use ground-truth, we do not need y^star, right?

\subsection{Soft Token-Level Alignment} 
MoverScore~\cite{zhao2019moverscore} is a recently 
%introduced 
proposed evaluation metric to measure 
the semantic similarity %distance 
between system outputs ($\mathbf{y}$) %translation 
and human references ($\mathbf{y}^\star$). 
%
It aligns semantically similar tokens from $\mathbf{y}$ and 
$\mathbf{y}^\star$ by minimizing the 
WMD. 
% \todo{YG: @Wei, check whether this is correct.}
%It implicitly aligns semantically similar words %and 
%by %finding the amount of flow traveling between them.\todo{SE: flow is too general} %these words. 
%determining the optimal transformation between two sets in terms of `transportation costs'. 
%Inspired by the success of MoverScore, 
%
Below, we extend MoverScore to the cross-lingual
case, so as to measure the semantic similarity between
$n$-grams in source text $\mathbf{x}$ and in system 
translation $\mathbf{y}$. 
%to compare semantic similarity between system translation and source text. 
%for comparing system output $\mathbf{y}$ to source text $\mathbf{x}$. 
%In the following, we formulate Cross-lingual MoverScore operating on $n$-grams.
% \todo{SE: let's use cross-lingual rather than multi-lingual}
% \todo{SE: some package appears to be missing here. See error messages.}

%Let $\bx$ and $\by$ be source sentence and system translation viewed as sequences of $n$-grams: $\bx^n$ and $\by^n$, i.e., $\bx_n = (\ervx_1^{n}, \dots, \ervx_m^{n})$. 
First,  we decompose $\mathbf{x}$ into a sequence $n$-grams, 
denoted by $\bx_n = (\ervx_1^{n}, \dots, \ervx_m^{n})$.
The same operation is applied to $\mathbf{y}$, and we
denote the resulting sequence as $\by_n$.
%
%then we define a distance metrix $C$ such that 
%If we have a Euclidean distance metric between $n$-grams,
% \todo{SE: $d$ has disappeared. $d=||\cdot||_2$?} 
Given $\bx_n$ and $\by_n$,
we can then define a distance matrix $\mC$ such that 
$\mC_{ij} =  \|E(\ervx^n_i) - E(\ervy^n_j) \|_2$ 
is the distance between the $i$-th $n$-gram of $\bx$ 
and the $j$-th $n$-gram of $\by$, 
where $E$ is a \emph{cross-lingual} embedding function that
maps $n$-grams in %disparate 
different languages to %their vector representations in 
a shared embedding space. 
%
In this work, we investigate %$E$ as 
the use of either cross-lingual aligned word embeddings (FastText~\cite{bojanowski2017enriching}) 
or multilingual contextualized embedding (Mutlilingual BERT~\cite{Devlin:2018}) as function  $E$.

The $\WMD$ between the two sequences of $n$-grams $\bx^n$ and $\by^n$ with associated $n$-gram weights $\f_{\bx^n}\in\R^{|\bx^n|}$ and $\f_{\by^n}\in\R^{|\by^n|}$ is then defined by:
\begin{align*}
& m(\bx,\by):= \WMD(\bx^n,\by^n)
= \min_{\mF} \sum_{ij} \mC_{ij}\cdot \mF_{ij}, \\
&\text{s.t. } \mF\1=\f_{\bx^n},\;\;\mF^{\intercal}\1=\f_{\by^n},
\end{align*}
where $\mF \in\R^{|\bx^n|\times |\by^n|}$ is a transportation matrix with $\mF_{ij}$ denoting the amount of flow traveling from 
%the $i$-th $n$-gram %YG: these too many hyphens do not help but instead confuse the readers;  
$\ervx^n_i$ to %in $\bx^n$ to the $j$-th $n$-gram 
$\ervy^n_j$.
%in $\by^n$. 

\subsection{Sentence-Level Semantic Similarity}

In addition to measuring semantic distance between %system translation and human reference 
$\mathbf{x}$ and $\mathbf{y}$ 
at word-level, one can also encode them into sentence representations with multilingual sentence encoders like LASER~\cite{artetxe2019massively} and USE~\cite{yang2019multilingual}, and then measure their cosine distance
%compute the distance between 
%two sentences in %disparate 
%distinct languages 
%with cosine similarity: %, denoted as:
\begin{align*}
m(\bx,\by) = 1 - \frac{E(\bx)^{\intercal} E(\by)}{ \|E(\bx) \| \cdot  \|E(\by) \|}.
\end{align*}
% \todo{YG: @Wei: NOTICE! you want distance, so should use cosine distance instead of cosine similarity, right? Hence I add the '1-' part}

\subsection{Improving Cross-Lingual Alignments}
\label{sec:cla}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{figures/alignment2.pdf}
\caption{\todo[inline]{SE: I suggest to remove this picture, as I do not believe the explanations are correct} PCA Visualization of sentence embeddings of source sentence in German and reference translation in English. In the initial sentence embedding space encoded from FastText,\todo{SE: FastText hasn't been discussed before. Before, you said the alignment is bad, but now the spaces are independent, i.e., there is no mapping} 
source and reference embeddings are not aligned. While they are seemingly aligned in the cross-lingual space encoded from LASER with an implicit bilingual dictionary populated by shared words/wordpieces across languages (middle), these embeddings are ill-aligned when zooming into individual instances (right), where source sentences  are often close to translationese (word-by-word translation) instead of reference translation. %, which is less preferred by human raters. 
Ideally, with post-hoc cross-lingual alignment, one can mitigate this misalignment by projecting source sentence into reference translation.}
 \label{fig:alignment_visualization}
\vspace{-0.15in}
\end{figure*} 
%resulting 


Multilingual contextualized embeddings %yielded 
% from multilingual contextualizers 
like Multilingual BERT and LASER are potentially `ill-aligned' in the shared vector space for the following two reasons. 
1) They learn the cross-lingual mapping by matching the tokens
that appear in both languages (e.g.\ punctuation or words
like `OK', `MBA' and 'iPhone'); 
because the number of shared tokens across languages
is usually very small compared to the full vocabulary size,
the mapping is %hardly 
expected to be imprecise for the majority of the tokens.\todo{SE: What about LASER?}
%from an implicit
% \todo{SE: you use -ly words wrongly. -ly words are adverbs or adjectives --- they relate to verbs or adjectives. This means that `implicitly' needs a verb or adjective which it modifies. But this is missing here} 
%bilingual dictionary constructed with shared tokens (words or subwords units) alone, resulting in less accurate %to align 
%mappings for the tokens that are not shared across languages; 
% do not utilize any explicitly bilingual dictionary to learn cross-lingual mapping, leading to less accurate alignment, especially for words and wordpieces that are not shared across languages; 
2) Tokens %across languages are often overly shared. 
shared across languages sometimes deliver completely different
semantic meanings: 
%incorrectly shared, when they have surface forms that coincide per chance. 
for example, the word `gift' 
%means very differently in German and Swedish('posion' in German and 'to get married' in Swedish), which leads to a misalignment between cross-lingual embeddings when taking these 'gift' in pairs as bilingual dictionary to learn cross-lingual mapping.
means `poison' in German while in English it means `present'
or `natural talent'.
%has a very different meaning in German (`poison') compared to English.
% \todo{SE: to me it's unclear a) what the first point means, 2) what you mean by misalignment. You use the term `alignment' all over the place, but it's usage appears ill-aligned to me (pun!). Alignment in vector space vs. alignment between two sequences -- these are two different senses of alignment.}
%\todo{SE: what is overly shared? Wei: rewrote} 
% lead to misalignment across languages. For example, the English word `xx' would also appear in the German corpus, but it should be preferably paired with `xx'. `xx' in German instead of itself.
% \todo{SE: this is presented like a hypothesis but it should be framed like a conclusion from our experiments, I think. Wei: rewrote. SE: still it is a result: ``they have problems'', rather than ``we want to see whether they have problems''}

\todo{YG: agree with SE's comment: I can hardly see
why 'ill-alignment' described above makes 
MultiLing-BERT prefer word-by-word translation.
Hence I leave the rest of this subsection un-touched.}
As illustrated in Figure \ref{fig:alignment_visualization}, the misalignment between cross-lingual embeddings implies that source sentence embeddings become close to word-by-word translations instead of (human) references.  
As a consequence, reference-free metrics building upon these embeddings are expected to have a strong preference for overly literal translations.\todo{SE: I doubt this interpretation. Could it be, instead, that there are two  phenomena going on simultaneously: bad matching between certain words (i.e., "Mann" is not close to the English "man") and a preference for very literal translation. A preference for literal translation is almost the opposite effect.} 
%resulting in reference-free metric showing strong preference in literal translation when combining ill-aligned cross-lingual embeddings. 
In this paper, we attempt to address this `biased'  preference %in MT reference-free evaluation 
by post-hoc alignments.
% with %initial 
% debiasing methods inspired by research efforts addressing vector space biases such as gender bias \cite{zhao-etal-2017-men,dev-phillips-2019,lauscher2019general}. 

\paragraph{Notation}
Let $\mD=\{(w_{\ell}^1,w_{k}^1), \dots, (w_{\ell}^n,w_{k}^n)\}$ be a set of 
%bilingual dictionary with either word or sentence pairs provided or unsupervisedly learned from $\ell_i$th and $\ell_j$th language corpus. 
matched word or sentence pairs from two different languages $\ell$ and $k$. 
We define a %debiasing 
re-mapping
function $f$ such that any $f(E(w_{\ell}))$ and $E(w_{k})$ are better aligned in a shared vector space.


% For instance, as proposed by Aldarmaki & Diab (2019), one
% method to perform alignment on contextualized representations is to first use word alignment pairs
% extracted from parallel corpora as a dictionary, learn an alignment matrix W based on it, and apply
% W back to the extracted representations.

% \paragraph{Generalized Bias-Direction Debiasing (GBDD)}
\paragraph{Cross-lingual Projection (CLP)}
Given $\ell$ and $k$, one can stack all vectors\todo{SE: are these word vectors? Contextualized ones? Are there not infinitely many?} to form matrices $\mX_{\ell}$ and $\mX_{k} \in \mathbb{R}^{n\times d}$. \citet{mikolov13} propose to learn a projection matrix $W \in \mathbb{R}^{d\times d}$, 
% such that $\mW \mX_{\ell_1}$ can approximate $\mX_{\ell_2}$, 
%with SGD optimizer,
denoted as:
% To find the optimal projection matrix $W \in \mathbb{R}^{d\times d}$,  proposed to solve the following optimization problem:
\begin{equation}
    \min_{\mW}  \| \mW \mX_{\ell} - \mX_{k} \|_2. \nonumber
\end{equation}
\citet{xing-etal-2015-normalized} %latter 
achieve further improvement on the task bilingual lexicon induction when restricting $W$ to an orthogonal matrix such that $W^T W=I$, which turns the optimization into the Procrustes problem \cite{schonemann1966generalized} 
% \todo{SE: what is the Procustes problem? Wei: added citation} 
with the following closed-form solution:
\begin{align} \label{eq:procrustes}
    \hat{W} & = UV^\intercal, 
    U\Sigma V^\intercal = \text{SVD}(X_{\ell}X_{k}^\intercal) \nonumber
\end{align}
where $\hat{W}$ denotes the optimal solution and SVD($\cdot$) stands for the singular value decomposition. 

\paragraph{Universal Misaligned Direction (UMD)}\todo{SE: is this the official name? It sounds like incorrect English...}
Inspired by \citet{dev-phillips-2019, lauscher2019general}, we exploit their approaches to identify the most informative
% bias
misaligned direction between representations of source and human references in the shared embedding space.
% the misalignment between the representations of 
% most informative bias direction such that 
% accounting for the misalignment in the cross-lingual embedding space.\todo{SE: again, alignment/misalignment is used too frequently here, and it is not well-specified}
Formally, given %a language pair 
$\ell$ and $k$, one can create individual misaligned vectors  $E(w_{\ell}^i)-E(w_{k}^i)$ for each bilingual dictionary pair in $\mD$. Then we can stack these individual vectors to form a matrix $\mQ\in \mathbb{R}^{n\times d}$, where $d$ is the embedding size. Let a universal vector $\bv_B$ be the top singular vector of $\mQ$, accounting for the most informative misaligned direction.
% \todo{SE: why has bias-direction a hyphen?}
%\todo{SE: a reference is needed. What is the dimensionality of Q? Wei: added}

Instead of subtracting the bias direction $v_B$ from all vectors $E(w_{\ell})$ and $E(w_k)$, one can orthogonally project them along its bias direction, denoted as:
\begin{equation}
f(E(w_{\ell})) = E(w_{\ell}) - \text{cos}(E(w_{\ell}), v_B)v_B. \nonumber
\end{equation}
% \todo{SE: in the original paper, it's a dot product, but here you normalize it to cosine Wei: this is mathematically correct version}
 
% \paragraph{Composition of re-mapping functions}

% Describe the operator $\circ$


% \citet{lauscher2019general} exploit this approach to attenuate gender bias in static embeddings, while \citet{aldarmaki-diab-2019-context} use it to learn cross-lingual mappings on contextualized embeddings for better performance gain in sentence translation retrieval. We apply it to learn better cross-lingual alignments by fixing ill-aligned cross-lingual embedding.\todo{SE: Are we incremental on Aldarmaki?}

% \paragraph{Debiasing Pipeline}
% \citet{lauscher2019general} show that composing debiasing models results in performance gains in attenuating gender bias. We exploit a similar debiasing pipeline to combine the above two debiasing models %seamlessly 
% in order to mitigate the misalignment between cross-lingual embeddings. For example, one can first debias ill-aligned embeddings by subtracting them\todo{SE: subtracting them sounds incorrect} from the most informative bias-direction and then project its resulting embedding to the target language embedding with orthogonal projection, denoted as:
% \begin{equation}
% f(E(w_{\ell})) = W^\intercal(E(w_{\ell}) - \text{cos}(E(w_{\ell}), v_B)v_B). \nonumber
% \end{equation}
% The presented models can
% be seamlessly composed with one another. For example, one can first debias embeddings by subtracting them from universal bias direction and then project its resulting embedding to the target language with orthogonal  projection.\todo{SE: copied from another paper?}
% \subsection{Lanugage Model} For measuring the linguistic quality (e.g., fluency) of system translation $y'$, %of MT systems, 
% %we evaluate it with language model, denoted by:
% we use a language model (LM): 
% % We evaluate translation quality of MT systems  with language model 
% \begin{align*}
%     \mathfrak{m}_2(y')= \sum_{i=1}^n \textrm{idf}(y_i')\log p(y'_i|y'_1,\dots,y'_{i-1})
%     % prod_i^n p(s_n|s_1,\dots,s_{n-1})
% \end{align*}
% where system translation $y'$ contains a sequence of words $(y'_1 ,\dots,y'_m )$, and $\textrm{idf}(y_i')$ is the IDF of word $y_i'$ computed from all translations in the corpus.
%\todo{$x_i$ is a source word?! How do we know the number of source words in $y'$ and $x$ are the same? Wei: sorry, it is a typo. Just fixed}

\subsection{Translationese}
% The illness of Cross-lingual Embeddings}
% Translatonese is a common phenomena in Machine Translation, which translates source sentence literally to the target language with fluency loss.
% the degree to which source sentence is literally translated
A strong MT metric should strongly prefer
%Desirable reference-free metrics should strongly prefer
(high quality) human references over %(bad forms of)
translationese (e.g., word-by-word translations). 
%for a source sentence input. %when comparing each of them against source sentence,
%while it also 
% In addition, a strong metric should 
% %They should likewise %show the indifference between fully code-switching translation (source sentence itself) and human reference. 
% prefer human references over a fully code-switching translations ($\mathbf{y}=\mathbf{x}$).
% \todo{YG: this so-called 'code-switching' translation
% is actually not a translation, because $\mathbb{y}$
% is in the same language as $\mathbf{x}$. As least
% for an outsider like me, I feel this is counter-intuitive.}
%To re-evaluate the reliability of reference-free metric in this line, we present two criteria, namely 
To measure a metric's ability to distinguish 
word-by-word translations and 
code-switching translations,
we define the 
W2W (word-by-word) 
% and CS (code-switching) 
statistics as follows: 
%to measure the degree to which each metric prefers literal and code-switching translation instead of human reference, denoted as:
\begin{align*}
\text{W2W} %(\mathbf{x},\mathbf{x}',\mathbf{y}^\star) 
&= \frac{1}{N}\sum_{(\mathbf{x},\mathbf{x}',\mathbf{y}^\star)} I(m(\mathbf{x}, \mathbf{y^\star}) < m(\mathbf{x}, \mathbf{x}'))\nonumber
% \\
% \text{CS} %(\mathbf{x},\mathbf{y}^\star) 
% % &= \frac{1}{N}\sum_{(\mathbf{x},\mathbf{y}^\star)} I(m(\mathbf{x}, \mathbf{y}^\star) >  m(\mathbf{x},\mathbf{x})) \nonumber
% &= \frac{1}{N}\sum_{(\mathbf{x},\mathbf{y}^\star)} (m(\mathbf{x},\mathbf{x}) - m(\mathbf{x}, \mathbf{y}^\star)) \nonumber
\end{align*}
%where $x$ and $z$ denote source sentence and human reference, $y$ denotes either word-by-word or code-switching translation, m is reference-free metric.
where $\mathbf{x}'$ is a naive (context-free) word-by-word translation of $\mathbf{x}$, 
$I(\cdot)$ is the indication function and
$1/N$ is used to normalize the value to
$[0,1]$.
%$N$ is the number of instances, and $I(\cdot)$ is the function that takes the value $1$ if its argument evaluates to true, and takes the value 0 otherwise. 
%Lower scores of both statistics are better.
For both statistics, a lower value means the metric
prefers references more often, hence suggests
better quality of the metric.

\paragraph{Language Model} 
%After re-evaluating 
%reference-free metrics, 
\citet{edunov-2019} show that BLEU often fails to %assessing 
capture the improved fluency of back-translations;
hence they propose to take a language model as 
the fluency scorer to complement BLEU.
In line with their method, 
%in reference-free evaluation, since reference-free metric potentially struggle in assessing the fluency of word-by-word and code-switching translation, 
we complement our cross-lingual models with a language model (trained on large monolingual corpus),  e.g., GPT~\cite{radford2018improving}. 
%as a fluency scorer. 
We assume the language model will help to penalize 
word-by-word and code-switching translations, 
hence boosting the performance of our metrics.
%
%This in particular addresses problems of overly literal translations or code-switching of which we suspect that cross-lingual metrics are susceptible to.   
%assessment to complement reference-free metric that in turn accounts for adequacy between source and system translation.

% We observe that debiasing cross-lingual embeddings can alleviate the ill-alignment in a shared bilingual space, but %they are 
% the embeddings still have problems 
% %hard 
% to fully discriminate either word-by-word or code-switching translations from human references. To this end, we also combine our reference-free metric with a language model like GPT, which takes into account 
% % the semantic similarity between source sentence and system translation as well as 
% the translation quality from linguistic perspective, denoted as:
% \begin{align*}
%     \mathfrak{m}(x,y) = \alpha_1 \mathfrak{m}_1(x,y) + \alpha_2 \text{LM}(y)
% \end{align*}
% \todo[inline]{SE: notation here is inconsistent}
% \todo[inline]{SE: Overall: We should not frame these things as results, because the results are discussed later. We should frame them as approaches. Wei: done}
% where we set $\alpha_1=1$ and $\alpha_2=0.05$ for all language pairs in our experiment.



% \paragraph{Cross-lingual Alignment} We investigate word- and sentence-level mapping to debias the misalignment between cross-lingual embeddings. Specifically, we attenuate the bias in cross-lingual word embedding space for FastText and Multilingual BERT as well as in the sentence embedding space for LASER and USE.

==> 4-experiments-removed-parts.tex <==
\begin{figure}
\begin{minipage}{0.49\linewidth}  
	\centerline{\includegraphics[width=\linewidth]{figures/de_en_CLDA_DA.pdf}}  
\end{minipage} 
\begin{minipage}{0.49\linewidth}  
	\centerline{\includegraphics[width=\linewidth]{figures/ru_en_CLDA_DA.pdf}}  
\end{minipage} 
 \caption{Correlation between CLDA and DA on two language pairs.
 }
 \label{fig:CLDA_DA}  
\vspace{-0.15in}
\end{figure} 

% \begin{figure}
% \begin{minipage}{0.49\linewidth}  
% 	\centerline{\includegraphics[width=\linewidth]{figures/de_en_CLDA_DA_metric.pdf}}  
% \end{minipage} 
% \begin{minipage}{0.49\linewidth}  
% 	\centerline{\includegraphics[width=\linewidth]{figures/ru_en_CLDA_DA_metric.pdf}}  
% \end{minipage} 
%  \caption{Correlation between reference-free metrics and DA versus CLDA.
%  }
%  \label{fig:CLDA_DA_metric}  
% \vspace{-0.15in}
% \end{figure} 
For each system translation, we collect segment- and system-level human judgments for evaluating the quality of our refernece-free metrics. The former judgments assigns one direct assessment (DA) score to each pair of system and human translations, while system-level judgments associate each system with a single DA score averaged on all pairs.
% assigning one direct assessment (DA) score to the system translation against reference.
However, a cross-lingual DA score, which we will call CLDA, which compares system translations against source is not provided. 
% This would be a discrepancy between what reference-free metrics can measure and DA judgments when evaluating reference-free metrics against DA instead of CLDA. 
This may pose a problem as we suspect that there is a mismatch between DA and CLDA because they compare system translation with different targets. To validate the suitability of DA in the reference-free evaluation,
% \todo{SE: we should add a few words about how translators improve references by simplification, e.g., https://arxiv.org/abs/1704.07146} %namely, 
% This may mean that cross-lingual 
% %reference-free 
% metrics correlate with CLDA better than with DA.
% To validate this hypothesis, 
we take two language pairs (de-en and ru-en) in WMT2017 test set, annotated for DA judgment, and ask two annotators who are proficient in English and native speakers in German and Russian to re-annotate it with CLDA assessments.
% re-annotate it with CLDA assessments  
% We opt for two language pairs (de-en and ru-en) to annotate, with two annotators for each pair who are proficient in English and native speakers in the source language.
% \todo{SE: the details are not yet correct, I think}. 
We follow the DA guidelines (e.g., 0-100 scale) but compare $\mathbf{y}$ against $\mathbf{x}$ instead of $\mathbf{y}^\star$.%human translation 
We observe that there is no such mismatch since they correlate moderately \footnote{The Pearson correlation between two annotators in de-en is 0.628 while 0.456 in ru-en.} with each other as shown in Figure in \ref{fig:CLDA_DA}. 
% \todo{YG: how about the correlation between the annotators' scores? In other words,
% how much agreement do annotators have? I ask this because ref-free metric should
% naturally correlate better than CLDA. Hence I suspect the quality of the CLDA 
% scores collected.}
% Indeed, Figure \ref{fig:CLDA_DA_metric} shows that evaluating reference-free metrics against DA judgment would overestimate the quality of these metrics as they often correlate worse with CLDA than with DA. However, it is valid to take DA as a surrograte of CLDA in reference-free evaluation when CLDA is not provided.\todo{SE: maybe drop the last two sentences and the figure. Not sure if we should report this.}

% \footnote{\cite{rankel-EtAl:2013:Short,novikova-etal-2017-need} show that metrics often correlate well with system-level human judgments}
% We follow the standard practice from WMT17 and WMT18 to report absolute Pearson correlation $|\rho|$ to evaluate metric quality on the newstest2017 test set and compute significance with the Williams test (Williams, 1959), while we report Kendall rank correlation $\tau$ on newstest2018 test set and compute significance with the bootstrap re-sampling for $\tau$ Graham & Baldwin (2014) \footnote{In WMT2018, DA
% judgements were converted to relative ranking judgements (daRR) due to insufficient number of judgements collected for each translation}.

==> introduction_old.tex <==
\section{Introduction}

\begin{enumerate}
    \item References are costly, we want to get rid of them
    \item References also limit evaluation to existing parallel data, which makes it difficult to estimate translation quality on new domains (e.g., poetry)
    \item Few works have addressed reference-free evaluation
    \item Older works ($<$ 2016) did not have good results
    \item Currently, strong monolingual evaluation models have been proposed as well as an array of multilingual encoders
    \item We explore whether these can solve the reference-free problem
    \item We also explore other approaches (Maxime, POSScore, DepScore)
    \item We find that
    \item (i) cross-lingual approaches need a LM
    \item (ii) can beat the SOTA
    \item (iii) current evaluation (DA(y,y') or HTER(x,y')) is flawed
    \item (iv) cross-lingual embeddings can be adversarially fooled and assign too high probability mass to literal translations (indicating that they are either more or less bag-of-words models or are sensitive to adversarial attacks) 
\end{enumerate}
